Using Generative Agents to Create Tip Sheets for Investigative Data Reporting

This paper introduces a system using generative AI agents to create tip sheets for investigative data reporting. Our system employs three specialized agents--an analyst, a reporter, and an editor--to collaboratively generate and refine tips from datasets. We validate this approach using real-world investigative stories, demonstrating that our agent-based system generally generates more newsworthy and accurate insights compared to a baseline model without agents, although some variability was noted between different stories. Our findings highlight the potential of generative AI to provide leads for investigative data reporting.

==> tables/3_evaluation.tex <==
\begin{table*}[t!]
  \caption{Evaluation of both setups on five selected stories}
  \label{tab:results}
  \centering
  \begin{tabular}{p{1.4cm}  p{1.2cm} rrr}
    \toprule
    Project & Model & Validity & Newsworthiness & Precision  \\
    \midrule
    \multirow[t]{4}{1.4cm}{\texttt{themarkup-\newline scoring}} & baseline  & 0.93 & 0.46 & 0.04 \\
    & agents & 0.90 & 0.70 & 0.13 \\
    \\
        \multirow[t]{4}{1.4cm}{\texttt{rferl- headlines}} & baseline & 0.57 & 0.40 & 0.33 \\ 
    & agents & 0.77 & 0.63 & 0.53 \\
    \\ 
        \multirow[t]{4}{1.4cm}{\texttt{civio- emergency}} & baseline & 1.00 & 0.63 & 0.40 \\
    & agents & 0.93 & 0.73 & 0.27 \\
    \\
        \multirow[t]{4}{1.4cm}{\texttt{netra- executions}} & baseline & 0.80 & 0.47 & 0.33 \\
    & agents & 0.87 & 0.63 & 0.57 \\
    \\
        \multirow[t]{4}{1.4cm}{\texttt{readr- ads}} & baseline & 0.80 & 0.47 & 0.27 \\
    & agents & 0.97 & 0.67 & 0.20 \\
\\
        \midrule
        \multirow[t]{4}{1.4cm}{Overall} & baseline & 0.82 & 0.52 & 0.28 \\
    & agents & \textbf{0.89} & \textbf{0.67} & \textbf{0.34} \\
    \bottomrule
  \end{tabular}
\end{table*}

